Supervisor Localization of Discrete-Event Systems with Infinite Behavior

Recently we developed supervisor localization, a top-down approach to distributed control of discrete-event systems (DES) with finite behavior. Its essence is the allocation of monolithic (global) control action among the local control strategies of individual agents. In this report, we extend supervisor localization to study the distributed control of DES with infinite behavior. Specifically, we first employ Thistle and Wonham's supervisory control theory for DES with infinite behavior to compute a safety supervisor (for safety specifications) and a liveness supervisor (for liveness specifications), and then design a suitable localization procedure to decompose the safety supervisor into a set of safety local controllers, one for each controllable event, and decompose the liveness supervisor into a set of liveness local controllers, two for each controllable event. The localization procedure for decomposing the liveness supervisor is novel; in particular, a local controller is responsible for disabling the corresponding controllable event on only part of the states of the liveness supervisor, and consequently, the derived local controller in general has states number no more than that computed by considering the disablement on all the states. Moreover, we prove that the derived local controllers achieve the same controlled behavior with the safety and liveness supervisors. We finally illustrate the result by a Small Factory example.

==> Subsec_ProductSys.tex <==

\subsection{Product Systems}

Let the plant ${\bf G}$ be comprised of $N$ ($N > 1$) component agents
\[{\bf G}_k = (Q_k, \Sigma_k, \delta_k, q_{k,0},\mathcal{G}_k) ~~ k = 1,..., N.\]
Here we assume that $\Sigma_k$ are pairwise disjoint, i.e. 
$\Sigma_k \cap \Sigma_j =\emptyset$ ($j \in [1,N]$) if $j \neq k$.
Then 
\begin{align}
{\bf G} = (Q, \Sigma, \delta, q_0, \mathcal{G})
\end{align} 
is the {\it synchronous product} of ${\bf G}^k$ ($k \in [1,N] := \{1,...,N\}$),
written as ${\bf G} := \mathop{||}\limits_{k \in [1,N]} {\bf G}_k$,
defined according to
\begin{align*}
~(i) ~&Q = \prod\limits_{k \in [1,N]} Q_k;\\
~(ii) ~&\Sigma = \mathop{\dot\bigcup}\limits_{k \in [1,N]} \Sigma_k;\\
~(iii) ~&q_0 = (q_{1,0},..., q_{N,0});\\
~(iv) ~&\delta((q_1,..., q_k, ..., q_N),\sigma) = (q_1, ..., \delta_k(q_k, \sigma),...,q_N) ~\text{provided $\delta_k(q_k,\sigma)!$}
\end{align*}


Let $L({\bf G}_k)$ and $S({\bf G}_k)$ be the finite and infinite
behaviors of ${\bf G}_k$ respectively; then the finite and
infinite behavior of $\bf G$ are
\begin{align*}
L({\bf G}) = \{s \in \Sigma^* | P_k(s) \in L({\bf G}_k), k \in \mathcal{K}\}\\
S({\bf G}) = \{s \in \Sigma^\omega | P_k(s) \in S({\bf G}_k), k \in \mathcal{K}\}
\end{align*}

% the end


==> Subsec_SupSynth.tex <==


\subsection{Effective Supervisor Synthesis} \label{Subsec:SupSynth}


To construct a supervisor $f^\omega$ described above, we need to compute $\sup\mathcal{C}^\omega(E)$ and $\inf\mathcal{F}^\omega(A)$
in advance. To that end, we assume that a deterministic Rabin-B\"{u}chi automaton
\begin{align} \label{eq:plant_Rabin}
\mathcal{A} = (Q, \Sigma, \delta, q_0, \{(R_p, I_p): p \in P\}, \mathcal{G})
\end{align}
is given, such that the $*$-automaton $(Q, \Sigma, \delta, q_0)$ accepts the
$*$-behavior $L({\bf G}) \subseteq \Sigma^*$ of ${\bf G}$, the B\"{u}chi automaton
$(Q, \Sigma, \delta, q_0, \mathcal{G})$ accepts the $\omega$-behavior
$S({\bf G}) \subseteq \Sigma^*$ of ${\bf G}$, and the Rabin automaton
$(Q, \Sigma, \delta, q_0, \{(R_p, I_p): p \in P\})$ accepts $E \subseteq \Sigma^\omega$
(such an automaton can be constructed from the DES model ${\bf G}$ in (\ref{eq:plant}) and a Rabin automata
accepting $E$).\footnote{If $S({\bf G})$ is $\omega$-closed, by Proposition 5.6 in \cite{Thistl91}
then it is redundant for the supervisor synthesis, and thus we can assume that
$S({\bf G}) = lim(S({\bf G}))$. In that case, it can be interpreted
as an absence of liveness assumptions in the modelling of the uncontrolled DES. Namely, in the DES
model ${\bf G}$ in (\ref{eq:plant}), we may drop the B\"{u}chi acceptance criterion,
Moreover, the computation of $\sup\mathcal{C}^\omega(E)$ is different with
that when the liveness assumptions is considered; for details, see \cite[Chapter 7]{Thistl91}.}

First, the computation of $\sup\mathcal{C}^\omega(E)$ begins with computing the {\it controllability
subset} $C^\mathcal{A} \subseteq Q$ of $\mathcal{A}$ in (\ref{eq:plant_Rabin}).
The subset $C^\mathcal{A}$, together with a map
\begin{align*}
\phi^{\mathcal{A}} : C^\mathcal{A} \rightarrow \Gamma
\end{align*}
defined on it, can be obtained by a subset construction algorithm \cite{ThiWon94a}
(recursively applying the fixpoint calculus method \cite{EmeLei86}).
%Here $\Gamma := \{\gamma \subseteq \Sigma| \gamma \supseteq \Sigma_{u}\}$ is as defined as previous.
By Theorem 8.12 in \cite{Thistl91}, the deterministic Rabin automaton
\begin{align} \label{eq:ASUP}
\mathcal{A}_{sup} = (Q, \Sigma, \delta, q_0, \{(R_p, I_p): p \in P\}) ~| ~C^\mathcal{A}
\end{align}
accepts the $\omega$-language $\sup\mathcal{C}^\omega(E)$. Here the operator `$|$', restriction
to a subset $C^\mathcal{A} \subseteq Q$, turns all other states into {\it degenerate}\footnote{A
state $q \in Q$ is {\it degenerate} if there are transitions leaving $q$ but all of them lead
back to $q$.} states that does not satisfy the Rabin acceptance
condition $\{(R_p, I_p): p \in P\}$. Note that $\mathcal{A}_{sup}$ is a
deterministic Rabin automaton because $\mathcal{A}$ is deterministic and
the operator `$|$' does not change this property.

Second, to compute $\inf\mathcal{F}^\omega(A)$, we have by Proposition 5.8 in \cite{Thistl91},
$\inf\mathcal{F}^\omega(A) = clo(A) \cap S({\bf G})$.
Given a deterministic Rabin automaton\footnote{Other $\omega$-automata including deterministic or nondeterministic
Rabin, B\"uautomaton can be converted into a deterministic Rabin automaton}
which accepts the $\omega$-language $A$, we construct a deterministic
Rabin automaton $\mathcal{A}_{inf}$ accepting $\inf\mathcal{F}^\omega(A)$ by:
first construct an $\omega$-automaton accepting $clo(A)$, and then
intersect it with $\bf G$ which accepts the $\omega$-language $S({\bf G})$.

Now that we have
\begin{enumerate}[(i)]
\item a deterministic Rabin automata $\mathcal{A}_{sup}$ accepting $\sup\mathcal{C}^\omega(E)$,
\item a controllability subset $C^{\mathcal{A}}$ together with a map $\phi^{\mathcal{A}} : C^\mathcal{A}
\rightarrow \Gamma$,
\item a deterministic Rabin automaton $\mathcal{A}_{inf}$ accepts
$\inf\mathcal{F}^\omega(A)$,
\end{enumerate}
we are able to check the existence of the supervisor $f^\omega$ and construct it if exists.

The existence verification of $f^\omega$ is equivalent to check the containment
$\inf\mathcal{F}^\omega(A) \subseteq \sup\mathcal{C}^\omega(E)$;
it suffices to test the automaton $\mathcal{A}_{inf} \slash \mathcal{A}_{sup}$
accepting $\inf\mathcal{F}^\omega(A)\slash\sup\mathcal{C}^\omega(E)$
for emptiness.\footnote{$\mathcal{A}_{inf} \slash \mathcal{A}_{sup}$ can be obtained
by intersect $\mathcal{A}_{inf}$ with the complement of $\mathcal{A}_{sup}$.}
When the answer is yes, $f^\omega$ is constructed as follows.

\begin{enumerate}[(i)]

\item Let ${\mathcal{A}}_{sup} = (Q', \Sigma, \delta', q_0', \{(R_p', I_p'): p \in P\})$ be the deterministic
Rabin automaton accepting $E' := \sup\mathcal{C}^\omega(E)$. Then a subset $Q_m' \subseteq Q'$ can be computed such
that the $*$-automaton $(Q_m', \Sigma, \delta', q_0')$ accepts $pre(E')$.
Because $E'$ is $*$-controllable with respect to ${\mathcal{A}}$,
we may define the map $\phi_0: Q_m' \rightarrow \Gamma$ as
\[\phi_0(q') := \{\sigma \in \Sigma| \delta(q',s\sigma) \in Q_m'\};\]
then by the proof of Proposition 4.4 \cite{Thistl91}, the map $f_0: \Sigma^* \rightarrow \Gamma$ given by
\[f_0^\omega(k) := \phi_0(\delta'(q_0',k))\]
is a complete, deadlock-free supervisor for $\mathcal{A}$ that synthesizes the
$*$-language $pre(E')$ and the $\omega$-language $clo(E')\cap S({\bf G})$.

\item For each $k \in pre(E')$, let $q = \delta'(q_0',k)$,
and let $\mathcal{A}_q = (Q', \Sigma, \delta', q, \{(R_p', I_p'): p \in P\})$.
Define $f_k^\omega: \Sigma^* \rightarrow \Gamma$ as
\[f_k^\omega(l/k) := \phi^{\mathcal{A}}(\delta'(q, l/k)),\]
where $\phi^{\mathcal{A}}: Q \rightarrow \Gamma$ is obtained in the process of computing the
controllability subset $C^{\mathcal{A}}$. It is shown in Theorem 5.9 \cite{Thistl91} that
$f_k^\omega: \Sigma^* \rightarrow \Gamma$ is a complete, deadlock-free supervisor
for $\mathcal{A}_q$, which synthesizes some $\omega$-sublanguage $E_k' \subseteq E'/k$
and $*$-sublanguage $pre(E_k')$.

\item Define the supervisor
\begin{align} \label{eq:sup_omega}
f^\omega:\Sigma^*\rightarrow \Gamma
\end{align}
according to:
\begin{eqnarray}
f^\omega(l) :=
\left\{
   \begin{array}{ll}
      f_0^\omega(l) & \text{if}~~ l \in pre(A), \notag\\
      f_k^\omega(l/k) & \text{if}~~ l \in k ~pre(E_k')~\text{where}~ k\in M \\
      \text{undefined} & \text{otherwise} \notag
   \end{array}
\right.
\end{eqnarray}
where $M$ is the set of all elements of $pre(E')\slash pre(\inf\mathcal{F}^\omega(A))$ of minimal length.
\end{enumerate}

Under the control of $f^\omega$, the closed-loop behavior of $\bf G$
can be represented by a deterministic B\"uchi automaton
${\bf G}^{f^\omega} = (X, \Sigma, \xi, x_0, \mathcal{G}_x)$ constructed by:
\begin{enumerate}[(i)]

\item Select $x_0 \in X$ corresponds to $q_0 \in Q$.

\item $\xi : X\times \Sigma \rightarrow X$ with $\xi(x,\sigma) = x'$
if there exists $s \in \Sigma^*$ such that $\xi(x_0, s)!$, $\delta(q_0,s\sigma)!$, and $\sigma \in f^\omega(s)$.

\item $\mathcal{G}_x := \{x \in X| (\exists s \in \Sigma^*)~ \xi(x_0, s) = x, \delta(q_0, s) \in \mathcal{G}\}$.
\end{enumerate}
%The finite and infinite behaviors of ${\bf G}^{f^\omega}$ are:
%\begin{align}
%L({\bf G}^{f^\omega}) &:= pre(\inf\mathcal{F}^\omega(A)) \cup \bigcup_{k\in M}k~ pre(E_k') \label{eq:sub1:implement}\\
%S({\bf G}^{f^\omega}) &:= \inf\mathcal{F}^\omega(A) \cup \bigcup_{k\in M}k~ E_k' \label{eq:sub2:implement}
%\end{align}

It is shown by \cite[Theorem 5.3]{ThiWon94b} that $f^\omega:\Sigma^*\rightarrow \Gamma$ defined above
is a complete, deadlock supervisor for $\bf G$, and the infinite controlled behaviors
of $\bf G$ satisfies the condition (\ref{eq:scpw}).

The supervisor $f^\omega:\Sigma^*\rightarrow \Gamma$ exercises its control action
depending on its observation on finite strings in $\Sigma^*$, and thus as in the supervisory control
for $*$-languages \cite{Wonham16a}, $f^\omega$ can be implemented by a *-automaton. Let
\begin{align}\label{eq:monosup}
{\bf SUP} := (X, \Sigma, \xi, x_0)
\end{align}
Namely $\bf SUP$ has the same transition structure and thus same finite behavior with ${\bf G}^{f^\omega}$,
i.e. $L({\bf SUP}) = L({\bf G}^{f^\omega})$.
It derives from $L({\bf G}^{f^\omega}) \subseteq L({\bf G})$ and
$S({\bf G}^{f^\omega}) := lim(L({\bf G}^{f^\omega})) \cap S({\bf G})$ (by \ref{eq:infcontrolbehaiv})
that $\bf SUP$ is an {\it implementation} of the supervisor $f^\omega$, i.e.
\begin{align}
L({\bf G}) \cap L({\bf SUP}) &= L({\bf G}^{f^\omega}) \label{eq:sub1:implement}\\
S({\bf G}) \cap lim(L({\bf SUP})) &= S({\bf G}^{f^\omega})\label{eq:sub2:implement}
\end{align}

%We also call $\bf SUP$ the {\it monolithic} supervisor for $\bf G$.
Note that $\bf SUP$ is not the unique implementation of the supervisor, for example we may
get a state-minimal supervisor $\bf MINSUP$ by the reduction algorithm in \cite{SuWon04}
which also satisfies conditions (\ref{eq:sub1:implement}) and (\ref{eq:sub2:implement}).


%% the end

